RecSys Challenge 2016: job recommendations based on preselection of offers and gradient boosting

We present the Mim-Solution's approach to the RecSys Challenge 2016, which ranked 2nd. The goal of the competition was to prepare job recommendations for the users of the website Xing.com. Our two phase algorithm consists of candidate selection followed by the candidate ranking. We ranked the candidates by the predicted probability that the user will positively interact with the job offer. We have used Gradient Boosting Decision Trees as the regression tool.

==> acknowledgments.tex <==
\section{Acknowledgements}

TODO
% ze robilismy to w ramach paal-poc


==> introduction.tex <==
\section{Introduction}
Recommender systems are becoming more and more popular on the Web.
Everywhere from online shops to video-streaming websites,
suggesting user items/offers/movies that he will be interested in
can increase the profits of the companies involved.
It is no different 

TODO
% nie jestem pewien czy to jest konieczne, proponuje napisac to na koniec:
%
% * znaczenie systemow rekemndacyjnych w e-commerce, reklamie internetowej, serwisach typu xing
% * rozwinac opis naszego rozwiazania: ze wazne byly feature'y, ze xgboost sobie swietnie z nimi radzil (TODO proponuje dokladniej wyspecyfikowac co tu ma byc jak bedziemy wiedzieli ile to ma miejsca zajac)
TODO na pewno tutaj jakies odwolania do bibliografii sa potrzebne


